Differentially Private Algorithms for Learning Mixtures of Separated Gaussians

Learning the parameters of Gaussian mixture models is a fundamental and widely studied problem with numerous applications. In this work, we give new algorithms for learning the parameters of a high-dimensional, well separated, Gaussian mixture model subject to the strong constraint of differential privacy. In particular, we give a differentially private analogue of the algorithm of Achlioptas and McSherry. Our algorithm has two key properties not achieved by prior work: (1) The algorithm's sample complexity matches that of the corresponding non-private algorithm up to lower order terms in a wide range of parameters. (2) The algorithm does not require strong a priori bounds on the parameters of the mixture components.

==> relatedwork.tex <==
\subsubsection{Non-Private Clustering/Learning Gaussian Mixtures}

\begin{enumerate}
    \item \cite{vw02}. Spherical Gaussians.
        $\|\mu_i-\mu_j\| > C\max\{\sigma_i,\sigma_j\}
        \times \left((k\log(d/w_{min}))^{1/4} +
        (\log(d/w_{min}))^{1/2}\right)$.
        $\Omega\left(\frac{d^3}{w_{min}^2}
        \left(\ln\frac{d}{w_{min}} +
        \ln\left(\max\limits_{i=1}^{k}\frac{|\mu_i|^2}
        {\sigma_i^2}\right)\right)\right)$ samples.
    \item \cite{ak05}. Non-spherical Gaussians.
        $\|\mu_i-\mu_j\| > \tilde\Omega\left(\sqrt{d}
        (\sigma_{i,max}+\sigma_{j,max})^2\right)$.
        $O\left(\frac{d^2k^2\log(kd^2)}{\delta^2w_{min}^6}\right)$
        samples.
    \item \cite{kk10}. $\|\mu_i-\mu_j\| > \tilde\Omega
        \left(\frac{k\sigma_{max}}{\sqrt{w_{min}}}\right)$.
        Needs $n = \poly\left(\tfrac{d}{w_{min}}\right)$
        samples.
    \item \cite{as12}. Clustering Mixture of Gaussian's.
        Standard deviation for component $r$ in any
        direction is\\ at most $\sigma_r$.
        $\|\mu_i-\mu_j\| \geq c\sigma_{max}\sqrt{k}
        \textrm{polylog}\left(\frac{d}{w_{min}}\right)$.
        $n \gg \frac{d}{w_{min}}$ samples.
    \item \cite{abhlmp18}. Near optimal sample complexity
        for mixtures. Provide LB and matching UB for
        general Gaussians. Provide a UB that matches
        previously known LB for axis-aligned Gaussians.
        Running time exponential in $k$ and $d$.
    \item \cite{ajos14}. Mixtures of spherical Gaussians.
        Polynomial time estimator. Number of samples:
        $$O\left(\frac{dk^9}{\alpha^4}
            \log^2\left(\frac{d}{\beta}\right)\right).$$
\end{enumerate}

\subsubsection{Private Clustering/Learning Gaussian Mixtures}

\begin{enumerate}
    \item \cite{ks18}. Points from $d$-dimensional
        ball of diameter $R$, centered at the origin.
        $$c\mathrm{OPT} + \poly\left(\log(n),
            \log\left(\frac{1}{\beta}\right),
            \log\left(\frac{1}{\delta}\right),
            d, \frac{1}{\eps}, k\right)R^2$$
        $k$-means cost with probability at
        least $1-\beta$.
    \item \cite{bdlmz17}. Points from $d$-dimensional
        ball of diameter.
        $d=\Omega\left(\textrm{polylog}(n)\right)$.
        $$\mathrm{polylog}(n)\mathrm{OPT} + \poly\left(\log(n),
            d, \frac{1}{\eps}, k\right)$$
        $k$-means cost. If $\|x_i\|_0 \leq s$ , we get,
        $$\mathrm{polylog}(n)\mathrm{OPT} + \poly\left(\log(n),
            \log(d), \frac{1}{\eps}, k\right)$$
        $k$-means cost.
    \item \cite{hl18}. Points from $d$-dimensional
        ball of diameter $1$.
        Dataset satisfies ``well separability'':
        $\Delta_{k}^2 \leq \phi^2 \Delta_{k-1}^2$.
        $\Delta_{k-1}^2 \geq \tilde{\Omega}\left(
        \frac{n^{11/20}k^{7/4}d^{3/4}}{\eps^{1/2}\phi^{4}}\right)$.
        Classifies within $O(\phi^2)$ Wasserstein distance.
        Number of samples needed is in
        $\tilde{\Omega}\left(\frac
        {k^{35/9}d^{5/3}}{\eps^{10/9}\phi^{80/9}}\right)$.
    \item \cite{nrs07}. Learns mixtures of spherical
        Gaussians when mixing weights are uniform, and
        the variance is known (and the same, I think).
    \item \cite{nsv16}. Solving the $1$-cluster
        problem on a finite space. If $n$ is the
        number of samples, we get $O(\sqrt{\log(n)})$
        approximation of the optimal radius.
    \item \cite{ns17}. Solving the $1$-cluster
        problem on a finite space. If $n$ is the
        number of samples, we get $O(1)$
        approximation of the optimal radius.
    \item \cite{fxzr17}. Solving $k$-means
        clustering with multiplicative error
        $$O(k\log(n)),$$
        and additive error
        $$\wt{O}\left(k^2\sqrt{d}\right).$$
\end{enumerate}


Throughout the discussion, we assume that for $d$ greater
than some absolute constant, the following inequality is
satisfied:
$$d \geq O\left(\log\left(\frac{dk\sigma_M\log(R/\delta)}
    {\alpha\beta\eps w_{min}\sigma_m}\right)\right).$$

